Learning Abstract Task Representations

A proper form of data characterization can guide the process of learning-algorithm selection and model-performance estimation. The field of meta-learning has provided a rich body of work describing effective forms of data characterization using different families of meta-features (statistical, model-based, information-theoretic, topological, etc.). In this paper, we start with the abundant set of existing meta-features and propose a method to induce new abstract meta-features as latent variables in a deep neural network. We discuss the pitfalls of using traditional meta-features directly and argue for the importance of learning high-level task properties. We demonstrate our methodology using a deep neural network as a feature extractor. We demonstrate that 1) induced meta-models mapping abstract meta-features to generalization performance outperform other methods by ~18% on average, and 2) abstract meta-features attain high feature-relevance scores.

==> stats/abs_friedman.tex <==
\begin{figure*}
\centering
\begin{tikzpicture}[xscale=1]
\node (Label) at (2.382773597138918, 0.7){\tiny{CD = 0.38}}; % the label
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black] (2.0,0.5) -- (2.765547194277836,0.5);
\foreach \x in {2.0, 2.765547194277836} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);
 
\draw[gray, thick](2.0,0) -- (6.0,0); 
\foreach \x in {2.0,4.0,6.0} \draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
\node (Label) at (2.0,0.2){\tiny{1}};
\node (Label) at (4.0,0.2){\tiny{2}};
\node (Label) at (6.0,0.2){\tiny{3}};
\node (Point) at (2.4266666666666667, 0){};\node (Label) at (0.5,-0.25){\scriptsize{abstract}}; \draw (Point) |- (Label);
\node (Point) at (5.786666666666666, 0){};\node (Label) at (6.5,-0.25){\scriptsize{traditional}}; \draw (Point) |- (Label);
\node (Point) at (3.7866666666666666, 0){};\node (Label) at (6.5,-0.55){\scriptsize{hybrid}}; \draw (Point) |- (Label);
\end{tikzpicture}
\caption{Nemenyi - abs friedman.csv}
\label{fig:nemenyi}
\end{figure*}


==> stats/abs_friedman_avg.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[xscale=1]
\node (Label) at (3.9138679856945897, 0.7){\tiny{CD = 1.91}}; % the label
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black] (2.0,0.5) -- (5.827735971389179,0.5);
\foreach \x in {2.0, 5.827735971389179} \draw[thick,color = black] (\x, 0.4) -- (\x, 0.6);
 
\draw[gray, thick](2.0,0) -- (6.0,0); 
\foreach \x in {2.0,4.0,6.0} \draw (\x cm,1.5pt) -- (\x cm, -1.5pt);
\node (Label) at (2.0,0.2){\tiny{1}};
\node (Label) at (4.0,0.2){\tiny{2}};
\node (Label) at (6.0,0.2){\tiny{3}};
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black](1.95,-0.25) -- (4.05,-0.25);
\draw[decorate,decoration={snake,amplitude=.4mm,segment length=1.5mm,post length=0mm},very thick, color = black](3.95,-0.4) -- (6.05,-0.4);
\node (Point) at (2.0, 0){};\node (Label) at (0.5,-0.65){\scriptsize{Abstract}}; \draw (Point) |- (Label);
\node (Point) at (6.0, 0){};\node (Label) at (6.7,-0.65){\scriptsize{Traditional}}; \draw (Point) |- (Label);
\node (Point) at (4.0, 0){};\node (Label) at (6.5,-0.95){\scriptsize{Hybrid}}; \draw (Point) |- (Label);
\end{tikzpicture}
\caption{Nemenyi - abs friedman avg.csv}
\label{fig:nemenyi}
\end{figure}

